Exploring the Benefits of Teams in Multiagent Learning

For problems requiring cooperation, many multiagent systems implement solutions among either individual agents or across an entire population towards a common goal. Multiagent teams are primarily studied when in conflict; however, organizational psychology (OP) highlights the benefits of teams among human populations for learning how to coordinate and cooperate. In this paper, we propose a new model of multiagent teams for reinforcement learning (RL) agents inspired by OP and early work on teams in artificial intelligence. We validate our model using complex social dilemmas that are popular in recent multiagent RL and find that agents divided into teams develop cooperative pro-social policies despite incentives to not cooperate. Furthermore, agents are better able to coordinate and learn emergent roles within their teams and achieve higher rewards compared to when the interests of all agents are aligned.

==> Submit/IJCAI-Submit/ResubmissionFile_contents/Reviews-IJCAI-2022.tex <==

View Reviews
Paper ID
4599
Paper Title
Exploring the Benefits of Teams in Multiagent Learning
Reviewer #1
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        This paper proposes a MARL approach that would take into account pre-grouping of agents in equal-sized teams. Reward is assumed to be equally distributed between team members. The authors show using experiments in two different domains that under certain conditions the cooperation between agents is enforced, either between teammates and not teammates. The experiments are carried out on Iterated Prisoner Dilemma and Cleanup games.
    2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
        The paper presents and discusses many interesting results regarding the social behavior of agents towards cooperation, coordination, labour division, and role learning.
        The proposal seems to be new, different from other MARL approaches. The experiments are done on different domains. The discussion of the results is detailed and interesting, while the conclusions are relevant.

        While interesting on its own, condition (4) shows that the incentive to cooperate is present if we interact frequently with a teammate. This is somehow an obvious conclusion.
    3. What opportunities are there to improve the paper?
        English language must be checked.
        p.2: "Agent seek to maximize"
        One comment however regards the description of the Cleanup game. While for IPD (clearly simpler scenario) the definition is clear, I couldn’t find a formal and precise description of the game. Moreover, the brief description from page 3 is confusing. For example, why does an agent need to turn left or right, while movement is explicitly defined in a certain direction? What are the sensing capabilities of the agent? What is a “punishing beam”? And so on …. I would have liked to see this somewhere. Currently there is a link to github repo, but in my opinion this is not an acceptable definition of the game.
    4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
        N/A
    5. Overall assessment.
        Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
    6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
        The method for computing he rewards is new. There is no a priori assumption about agent preferences / profiles / strategies. The agents learn pro-social behavior only by fair interaction with others, teammates or not. The discussion of experiments is good and the conclusions are relevant.
    7. Are the results in this paper easily reproducible ?
        CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
    8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
        N/A

Reviewer #2
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        This paper explores the effects of explicit teams on homogeneous agents in social dilemma environments (iterated prisoner's dilemma and "cleanup" (the one with the dirty river and the apples), with evenly shared team rewards. Even with this fairly minimal definition of "team", multiple agent teams learn to do better using standard MARL techniques (deep Q-learning for IPD and PPO for Cleanup).
    2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
        The paper is clearly written, and straightforward even without referring to the appendices. A lot of work in MARL on cooperation tends to ignore the long tradition of work in the area pre-MARL, and this paper makes some nods to these classic conceptualizations (but, see below). Reproducibility is credible here, as the general ideas are clearly stated, the environments are fairly well-known, (although see below
    3. What opportunities are there to improve the paper?
        Nice to talk about at least a couple of classic team conceptualizations, but there really is nothing in the ideas tested that truly has the conceptualization of SharedPlans, Steam (based on Cohen & Levesque's formal teamwork model), or others more recent (e.g. DARPA Coordinators, etc.)
        Wonder if the specific MARL algorithm matters a lot, or just the way the teams are conceptualized.
        Questions of roles in the Cleanup problem are shown abstractly across the "society" and not team-by-team, although the authors do discuss that one team learns to freeload (in itself a second-level organizational structure perhaps)
        In all, the work is an initial result, as the paper raises many questions--however in the length required one really cannot deal with many more of them in any adequate way, so I would not fault them too much for that.
    4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
        How much do you feel that the cooperative responses to non-teammates that give the results such a boost are just a side effect of the limited representation in a MARL system---agents don't explicitly reason about action choice, but simply average the value of actions (via the q-update or other value computation explicit or implicit in most RL approaches)?
    5. Overall assessment.
        Weak accept. Useful. A good paper. The results and insights will benefit the field. I believe it should be accepted.
    6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
        Paper is clearly written, does not overreach, credibly reproducible, re-introducing at least in a very simple way, ideas that have been very well developed but set aside (for no particularly good reason, usually...)
    7. Are the results in this paper easily reproducible ?
        CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
    8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
        no, in fact the authors try to analyze things like differential effects on agents within teams.

Reviewer #3
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        In the context of multi-agent reinforcement learning (MARL) the paper explores how teams structures can achieve higher rewards than with aligned agents. The proposed model is evaluated using two complex social dilemmas from multi-agent RL (Iterated Prisoner's Dilemma, and the Cleanup Markov Game).
    2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
        This paper provides an original contribution :
        - it explores links between organizational psychology and AI
        - it shows benefits of teams in Multiagent Learning problems, from empirical evaluation using complex social dilemmas that are popular in recent multiagent RL.
    3. What opportunities are there to improve the paper?
        - I would appreciate Section 6 includes a discussion about how best team structures can emerge or be learned (ie. in future work) (see Question 1 below).
        - While remarks in Section 7 are interesting, I don't think it is necessary to add a specific short "Ethics Statement" section, after Discussion and Future Work. I think this should be incorporated into Section 6.
    4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
        I have questions that do not require providing new results :
        1) In the discussion section, I think there is a missing important question : while interest of team structures has been demonstrated, how to obtain the emergence of the best team structure ? How to learn such an efficient structure ?
        2) Did you explored other multi-agent problem, or other social dilemmas, in order to expand the study to generalize your results ? Or which ones do you expect to study ?
    5. Overall assessment.
        Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
    6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
        - The paper addresses an important problem in multi-agent systems, concerning the general methodology of multiagent learning (MARL), by examining how it is impacted by team structures.
        - The paper open new perspectives in MARL by bringing together OP (Organizational Psychology) and RL.
        - The paper is well written and the proposed model well formalized.
        - Experimental results are convincing with a good analysis.
        - The supplementary material is relevant and useful (eg. to present the Cleaning dilemma).
    7. Are the results in this paper easily reproducible ?
        CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
    8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
        No problem.

Reviewer #4
Questions

    1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
        The paper applies team formation to multi-agent reinforcement learning in the attempt to investigate whether team formation bring benefits to RL itself.
        Authors motivate the need to consider team formation in MARL, then present their model, and finally evaluate their approach in two benchmark problems: iterated prisoner's dilemma and cleanup game. The empirical evaluation reported in the manuscript fully support authors' claim that team formation brings better average global rewards, even w.r.t.\ fully-cooperative scenarios.
    2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
        - the paper is well written, well structured, easy to follow, and accessible to a large audience. It is a great pleasure to read the paper.
        - the empirical evaluation is very well thought and goes deep in explaining results.
    3. What opportunities are there to improve the paper?
        I think only one things could be improved: reproducibility of results.
        As the authors populate the supplementary material (not the main body of text) with details regarding implementation of the scenarios, and the empirical evaluation clearly shows that experiment have been implemented, why not sharing the code publicly?
        This would be even more important than usual also considering the explorative and pioneering work authors do, that is, analysing the effect of team formation theory in MARL.
    4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
        1) if teammates share rewards equally isn't there the risk of free-riding?
    5. Overall assessment.
        Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
    6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
        I am not expert in the field of team formation nor MARL, although I do have a general understanding of the research area and models and techniques.
        However, I believe the paper to be very well written, with a set of convincing points made during evaluation, and offering a breath of new air in MARL.
    7. Are the results in this paper easily reproducible ?
        CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
    8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
        no ethical concerns. I also suggest authors to remove their ethical section, as usually you want to put there something about human involvement in experiments or sensitive data, which is not your case.
        

==> Submit/IJCAI-Submit/Reviews-Rebuttals/rebuttal_draft.tex <==


REBUTTAL QUESTIONS

4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.


REVIEWER 2: 

Q: How much do you feel that the cooperative responses to non-teammates that give the results such a boost are just a side effect of the limited representation in a MARL system---agents don't explicitly reason about action choice, but simply average the value of actions (via the q-update or other value computation explicit or implicit in most RL approaches)?

% (A1) Review 2, Question 1: Thanks for asking this question, this is a very good observation. It is true that MARL agents simply average the value of actions to learn behaviors; however, the average (or expected) payoffs in the IPD for cooperation are often still less than for defection in many of our settings (i.e., defection would be the expected behavior of MARL agents). Instead, we see agents learn to cooperate even when they do not interact with their teammates enough to change the expected payoff and make cooperation have higher expected value. Although agents do not explicitly reason about their actions, the behavior is unexpected even for MARL systems.

(A2) Review 2, Question 1: This is a great question, thanks for asking it. You are correct that RL agents do not explicitly reason about their actions, but instead average some value associated with those actions. We are not sure to the theoretical extent of how or why teams help agents learn; however, we hypothesize that it could have an impact in both scenarios. Our main intuition is that teams reduce the penalty when agents act poorly while also reducing the distinction when agents receive high reward. This clearly impacts the learning mechanism in model-free RL and would surely be able to expand to scenarios where agents reason over actions, so long as their reasoning is informed by some type of feedback loop. This would be an interesting topic of further exploration.
 

REVIEWER 3:

Q1) In the discussion section, I think there is a missing important question : while interest of team structures has been demonstrated, how to obtain the emergence of the best team structure ? How to learn such an efficient structure ?

(A) Review 3, Question 1: Great question. This is something that is definitely worth further exploration! We identify two ways of how team emergence or structure could be learned: decentralized and centralized. The decentralized setting requires problems of negotiation and commitment, important research topics in multiagent systems. The centralized method could learn using structures inspired by hierarchical reinforcement learning, where multiple ``levels" of agents interact through feedback signals. Both settings are extremely different problems, but are both interesting and important given our research on teams.



Q2) Review 3, Question 2: Did you explored other multi-agent problem, or other social dilemmas, in order to expand the study to generalize your results ? Or which ones do you expect to study ?

(A) Review 3, Question 2: We focused on IPD and Cleanup since these are two well-studied environments, where cooperation is known to be challenging due to the structure of the social dilemma. We plan to expand our work beyond these environments, exploring other social dilemmas, environments with stochastic rewards, and hopefully, the role of team structures in sports. We have not yet made our code public to respect the anonymity requirements of the conference; however, we hope to make our code publicly available in the not too distant future to assist others and expand the study of multiagent teams.



REVIEWER 4:

Q1) if teammates share rewards equally isn't there the risk of free-riding?

(A) Review 4, Question 1: Good question. There are two types of potential free-riding.  First, free-riding between teammates since they will always receive the same reward (based on our definition of $TR_i$). Role specialization is different than free-riding since the roles in the case of Cleanup are interdependent. If an agent does not execute their role, this would be a type of free-riding between teammates; however, we do not observe this in our experiments. Agents optimizing for goals other than just their team's reward could lead to interesting behavior and is worth further exploration. Second, free riding between-teams is also a possibility and we do observe it in the 3/2 team structure of Cleanup (Team 1 only picks apples). This does involve a second-order coordination problem between teammates when conforming to the free-riding behavior towards other teams.


==> Submit/IJCAI-Submit/Reviews-Rebuttals/reviews.tex <==



Reviewer #1
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
This paper proposes a MARL approach that would take into account pre-grouping of agents in equal-sized teams. Reward is assumed to be equally distributed between team members. The authors show using experiments in two different domains that under certain conditions the cooperation between agents is enforced, either between teammates and not teammates. The experiments are carried out on Iterated Prisoner Dilemma and Cleanup games.
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
The paper presents and discusses many interesting results regarding the social behavior of agents towards cooperation, coordination, labour division, and role learning. 
The proposal seems to be new, different from other MARL approaches. The experiments are done on different domains. The discussion of the results is detailed and interesting, while the conclusions are relevant.

While interesting on its own, condition (4) shows that the incentive to cooperate is present if we interact frequently with a teammate. This is somehow an obvious conclusion.
3. What opportunities are there to improve the paper?
English language must be checked.
p.2: "Agent seek to maximize"
One comment however regards the description of the Cleanup game. While for IPD (clearly simpler scenario) the definition is clear, I couldn’t find a formal and precise description of the game. Moreover, the brief description from page 3 is confusing. For example, why does an agent need to turn left or right, while movement is explicitly defined in a certain direction? What are the sensing capabilities of the agent? What is a “punishing beam”? And so on …. I would have liked to see this somewhere. Currently there is a link to github repo, but in my opinion this is not an acceptable definition of the game. 
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
N/A
5. Overall assessment.
Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
The method for computing he rewards is new. There is no a priori assumption about agent preferences / profiles / strategies. The agents learn pro-social behavior only by fair interaction with others, teammates or not. The discussion of experiments is good and the conclusions are relevant.
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
N/A


****************************************************************************
****************************************************************************

Reviewer #2
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
This paper explores the effects of explicit teams on homogeneous agents in social dilemma environments (iterated prisoner's dilemma and "cleanup" (the one with the dirty river and the apples), with evenly shared team rewards. Even with this fairly minimal definition of "team", multiple agent teams learn to do better using standard MARL techniques (deep Q-learning for IPD and PPO for Cleanup).
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
The paper is clearly written, and straightforward even without referring to the appendices. A lot of work in MARL on cooperation tends to ignore the long tradition of work in the area pre-MARL, and this paper makes some nods to these classic conceptualizations (but, see below). Reproducibility is credible here, as the general ideas are clearly stated, the environments are fairly well-known, (although see below
3. What opportunities are there to improve the paper?
Nice to talk about at least a couple of classic team conceptualizations, but there really is nothing in the ideas tested that truly has the conceptualization of SharedPlans, Steam (based on Cohen & Levesque's formal teamwork model), or others more recent (e.g. DARPA Coordinators, etc.)
Wonder if the specific MARL algorithm matters a lot, or just the way the teams are conceptualized.
Questions of roles in the Cleanup problem are shown abstractly across the "society" and not team-by-team, although the authors do discuss that one team learns to freeload (in itself a second-level organizational structure perhaps)
In all, the work is an initial result, as the paper raises many questions--however in the length required one really cannot deal with many more of them in any adequate way, so I would not fault them too much for that.
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
How much do you feel that the cooperative responses to non-teammates that give the results such a boost are just a side effect of the limited representation in a MARL system---agents don't explicitly reason about action choice, but simply average the value of actions (via the q-update or other value computation explicit or implicit in most RL approaches)?
5. Overall assessment.
Weak accept. Useful. A good paper. The results and insights will benefit the field. I believe it should be accepted.
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
Paper is clearly written, does not overreach, credibly reproducible, re-introducing at least in a very simple way, ideas that have been very well developed but set aside (for no particularly good reason, usually...)
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
no, in fact the authors try to analyze things like differential effects on agents within teams.


****************************************************************************
****************************************************************************


Reviewer #3
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
In the context of multi-agent reinforcement learning (MARL) the paper explores how teams structures can achieve higher rewards than with aligned agents. The proposed model is evaluated using two complex social dilemmas from multi-agent RL (Iterated Prisoner's Dilemma, and the Cleanup Markov Game).
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
This paper provides an original contribution :
- it explores links between organizational psychology and AI
- it shows benefits of teams in Multiagent Learning problems, from empirical evaluation using complex social dilemmas that are popular in recent multiagent RL.
3. What opportunities are there to improve the paper?
- I would appreciate Section 6 includes a discussion about how best team structures can emerge or be learned (ie. in future work) (see Question 1 below).
- While remarks in Section 7 are interesting, I don't think it is necessary to add a specific short "Ethics Statement" section, after Discussion and Future Work. I think this should be incorporated into Section 6.
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
I have questions that do not require providing new results :
1) In the discussion section, I think there is a missing important question : while interest of team structures has been demonstrated, how to obtain the emergence of the best team structure ? How to learn such an efficient structure ?
2) Did you explored other multi-agent problem, or other social dilemmas, in order to expand the study to generalize your results ? Or which ones do you expect to study ?
5. Overall assessment.
Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
- The paper addresses an important problem in multi-agent systems, concerning the general methodology of multiagent learning (MARL), by examining how it is impacted by team structures.
- The paper open new perspectives in MARL by bringing together OP (Organizational Psychology) and RL.
- The paper is well written and the proposed model well formalized.
- Experimental results are convincing with a good analysis. 
- The supplementary material is relevant and useful (eg. to present the Cleaning dilemma).
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
No problem.


****************************************************************************
****************************************************************************



Reviewer #4
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
The paper applies team formation to multi-agent reinforcement learning in the attempt to investigate whether team formation bring benefits to RL itself.
Authors motivate the need to consider team formation in MARL, then present their model, and finally evaluate their approach in two benchmark problems: iterated prisoner's dilemma and cleanup game. The empirical evaluation reported in the manuscript fully support authors' claim that team formation brings better average global rewards, even w.r.t.\ fully-cooperative scenarios.
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
- the paper is well written, well structured, easy to follow, and accessible to a large audience. It is a great pleasure to read the paper.
- the empirical evaluation is very well thought and goes deep in explaining results.
3. What opportunities are there to improve the paper?
I think only one things could be improved: reproducibility of results.
As the authors populate the supplementary material (not the main body of text) with details regarding implementation of the scenarios, and the empirical evaluation clearly shows that experiment have been implemented, why not sharing the code publicly?
This would be even more important than usual also considering the explorative and pioneering work authors do, that is, analysing the effect of team formation theory in MARL.
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
1) if teammates share rewards equally isn't there the risk of free-riding?
5. Overall assessment.
Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
I am not expert in the field of team formation nor MARL, although I do have a general understanding of the research area and models and techniques.
However, I believe the paper to be very well written, with a set of convincing points made during evaluation, and offering a breath of new air in MARL.
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
no ethical concerns. I also suggest authors to remove their ethical section, as usually you want to put there something about human involvement in experiments or sensitive data, which is not your case.
Reviewer #2
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
This paper explores the effects of explicit teams on homogeneous agents in social dilemma environments (iterated prisoner's dilemma and "cleanup" (the one with the dirty river and the apples), with evenly shared team rewards. Even with this fairly minimal definition of "team", multiple agent teams learn to do better using standard MARL techniques (deep Q-learning for IPD and PPO for Cleanup).
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
The paper is clearly written, and straightforward even without referring to the appendices. A lot of work in MARL on cooperation tends to ignore the long tradition of work in the area pre-MARL, and this paper makes some nods to these classic conceptualizations (but, see below). Reproducibility is credible here, as the general ideas are clearly stated, the environments are fairly well-known, (although see below
3. What opportunities are there to improve the paper?
Nice to talk about at least a couple of classic team conceptualizations, but there really is nothing in the ideas tested that truly has the conceptualization of SharedPlans, Steam (based on Cohen & Levesque's formal teamwork model), or others more recent (e.g. DARPA Coordinators, etc.)
Wonder if the specific MARL algorithm matters a lot, or just the way the teams are conceptualized.
Questions of roles in the Cleanup problem are shown abstractly across the "society" and not team-by-team, although the authors do discuss that one team learns to freeload (in itself a second-level organizational structure perhaps)
In all, the work is an initial result, as the paper raises many questions--however in the length required one really cannot deal with many more of them in any adequate way, so I would not fault them too much for that.
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
How much do you feel that the cooperative responses to non-teammates that give the results such a boost are just a side effect of the limited representation in a MARL system---agents don't explicitly reason about action choice, but simply average the value of actions (via the q-update or other value computation explicit or implicit in most RL approaches)?
5. Overall assessment.
Weak accept. Useful. A good paper. The results and insights will benefit the field. I believe it should be accepted.
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
Paper is clearly written, does not overreach, credibly reproducible, re-introducing at least in a very simple way, ideas that have been very well developed but set aside (for no particularly good reason, usually...)
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
no, in fact the authors try to analyze things like differential effects on agents within teams.
Reviewer #3
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
In the context of multi-agent reinforcement learning (MARL) the paper explores how teams structures can achieve higher rewards than with aligned agents. The proposed model is evaluated using two complex social dilemmas from multi-agent RL (Iterated Prisoner's Dilemma, and the Cleanup Markov Game).
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
This paper provides an original contribution :
- it explores links between organizational psychology and AI
- it shows benefits of teams in Multiagent Learning problems, from empirical evaluation using complex social dilemmas that are popular in recent multiagent RL.
3. What opportunities are there to improve the paper?
- I would appreciate Section 6 includes a discussion about how best team structures can emerge or be learned (ie. in future work) (see Question 1 below).
- While remarks in Section 7 are interesting, I don't think it is necessary to add a specific short "Ethics Statement" section, after Discussion and Future Work. I think this should be incorporated into Section 6.
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
I have questions that do not require providing new results :
1) In the discussion section, I think there is a missing important question : while interest of team structures has been demonstrated, how to obtain the emergence of the best team structure ? How to learn such an efficient structure ?
2) Did you explored other multi-agent problem, or other social dilemmas, in order to expand the study to generalize your results ? Or which ones do you expect to study ?
5. Overall assessment.
Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
- The paper addresses an important problem in multi-agent systems, concerning the general methodology of multiagent learning (MARL), by examining how it is impacted by team structures.
- The paper open new perspectives in MARL by bringing together OP (Organizational Psychology) and RL.
- The paper is well written and the proposed model well formalized.
- Experimental results are convincing with a good analysis. 
- The supplementary material is relevant and useful (eg. to present the Cleaning dilemma).
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
No problem.
Reviewer #4
Questions

1. Please briefly summarize the main contributions of the paper in your own words. (Please do not include your evaluation of the paper here).
The paper applies team formation to multi-agent reinforcement learning in the attempt to investigate whether team formation bring benefits to RL itself.
Authors motivate the need to consider team formation in MARL, then present their model, and finally evaluate their approach in two benchmark problems: iterated prisoner's dilemma and cleanup game. The empirical evaluation reported in the manuscript fully support authors' claim that team formation brings better average global rewards, even w.r.t.\ fully-cooperative scenarios.
2. What are the main strengths of the paper? Please focus on novelty, soundness, significance and impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility (as specified in our reproducibility guidelines).
- the paper is well written, well structured, easy to follow, and accessible to a large audience. It is a great pleasure to read the paper.
- the empirical evaluation is very well thought and goes deep in explaining results.
3. What opportunities are there to improve the paper?
I think only one things could be improved: reproducibility of results.
As the authors populate the supplementary material (not the main body of text) with details regarding implementation of the scenarios, and the empirical evaluation clearly shows that experiment have been implemented, why not sharing the code publicly?
This would be even more important than usual also considering the explorative and pioneering work authors do, that is, analysing the effect of team formation theory in MARL.
4. What pressing questions do you have for the authors in the rebuttal ? List (and number) only questions about specific issues here that 1) could directly influence your evaluation of the paper, and 2) do not require providing new results. Typical questions include requests to clarify or justify particular issues, or about important relationships to other works.
1) if teammates share rewards equally isn't there the risk of free-riding?
5. Overall assessment.
Clear Accept. Interesting. A very good submission. I learned a lot from this paper. I vote and argue for acceptance. (Top 50% of accepted IJCAI papers.)
6. Justify your score in a few lines. Please focus on novelty, soundness, significance, expected impact, relevance to AI, clarity of exposition, and credibility with regard to reproducibility.
I am not expert in the field of team formation nor MARL, although I do have a general understanding of the research area and models and techniques.
However, I believe the paper to be very well written, with a set of convincing points made during evaluation, and offering a breath of new air in MARL.
7. Are the results in this paper easily reproducible ?
CREDIBLE: I believe that the obtained results can, in principle, be reproduced. Even though key resources (e.g., proofs, code, data) are unavailable at this point, the key details (e.g., proof sketches, experimental setup) are sufficiently well described for an expert to confidently reproduce the main results, if given access to the missing resources.
8. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted? Papers with a yes here will undergo additional ethical screening by senior members of the program committee. In case of glaring violations of well accepted ethical principles, IJCAI-ECAI 2022 reserves the right to reject the submission. Please check our Ethics Policy in the Call for papers for more details.
no ethical concerns. I also suggest authors to remove their ethical section, as usually you want to put there something about human involvement in experiments or sensitive data, which is not your case.









META REVIEW:

META-REVIEWER #23

META-REVIEW QUESTIONS

2. Summary of the discussion amongst the PC members.
There was a very short discussion on this paper because all the reviews were very positive and the PC members were happy with the rebuttal.
3. Reasons to accept.
The paper presents and discusses many interesting results regarding the social behavior of agents towards cooperation, coordination, labour division, and role learning.
The proposal is novel, different from other MARL approaches. 
The empirical evaluation is very well thought and goes deep in explaining results.
The conclusions are relevant.
Reproducibility is credible.
The paper is well written, well structured, easy to follow, and accessible to a large audience.
4. Reasons to reject.
None was brought up.
6. Independent of your judgement of the quality of the work, are there any ethical concerns with regard to responsible research or potential negative societal impacts of this submission that must be considered by IJCAI-ECAI 2022 before the paper can be accepted?
No

==> eq_analysis.tex <==

% \subsection{Equilibrium Analysis of IPD with Teams}

% \todo{Expected length: $\frac{1}{2}$ column.}

% This section will show calculations for how equilibrium changes from selfish IPD to system IPD.
% Teams shift the value of expected valuable action to interaction techniques.

% As discussed in Section \ref{sec:teams_model}, agents are bounded with their team through common-interest.


Given the existence of teams, agents are aware that they are either playing the game in Table~\ref{tab:pd_table} or Table~\ref{tab:pd_team}. 
% However, in the extreme case they may not be aware as to whether they are playing against a team member or not.
% Under these constraints w
We are interested in understanding whether cooperation can be supported in equilibrium and to this end we consider an iteration of the game.
Assume a pair of agents, $i,j$, have been selected to interact at some iteration of the IPD game. 
Furthermore, assume that agent $i$ knows that it will be matched to a teammate with probability $\inteam$ and a non-teammate with probability $(1-\inteam)$. 


% If agent $i$ decides to cooperate ($C$), its expected utility after algebraic simplification, subject to agent $j$'s strategy, is:
% \begin{align}
%     \mathbb{E}(C,\sigma_{T}) &= \frac{\inteam (b-c)(\sigma_{j,i}+1)}{2}+ (1-\inteam)(\sigma_{j,j} b-c).
%     \label{eq:team_coop}
% \end{align}
% If agent $i$ decides to defect ($D$), its expected utility after algebraic simplification, subject to agent $j$'s strategy, is:

% \begin{align}
%     \mathbb{E}(D,\sigma_{T}) &= \frac{\inteam \sigma_{j,i}(b-c)}{2} +(1-\inteam)\sigma_{j,j} b.
%     \label{eq:team_def}
% \end{align}

We calculate the expected utilities of cooperation and defection subject to $j$'s expected strategy profile, $\sigma_{T}$, in Appendix B and determine the conditions under which agent $i$ has incentive to cooperate as when $\mathbb{E}(C,\sigma_{T})\geq  \mathbb{E}(D,\sigma_{T})$.
% the expected value of cooperation is greater than defection subject to $\sigma_{T}$.
% This will occur whenever
% \begin{align}
%     \mathbb{E}(C,\sigma_{T})\geq  \mathbb{E}(D,\sigma_{T}). 
%     \label{eq:teams_constraint}
% \end{align}
% Instantiating Constraint~\ref{eq:teams_constraint} with Equations~\ref{eq:team_coop} and~\ref{eq:team_def} and simplifying we obtain that agent $i$ is best off cooperating when
Substituting in our derived expected values, we determine the environmental conditions when cooperation is incentivized as being when:
\begin{align}
    \inteam \geq \frac{2c}{b+c},
    \label{eq:final_requrement}
\end{align}
regardless of $\sigma_{T}$.
Since $b>c>0$, this constraint is meaningful. 
% \Kate{We can add the algebra in the appendix. Dave, can you add some more text as to why this is interesting? Sort of like what you had before.}
Satisfying Equation~\ref{eq:final_requrement} shifts the Nash Equilibrium of the social dilemma from ($D$, $D$) to ($C$, $C$).
% Agents do not explicitly interact in Cleanup, therefore the incentive structure is not able to be theoretically derived.




\begin{comment}
In previous work, common interest is typically modeled through reward sharing between agents~\cite{McKee2020SocialDA,Fu2019DeepMR,Leibo2019MalthusianRL,Hughes2018InequityAI,Durugkar2020BalancingIP}.
% Without knowing opponent strategies, this means the expected values of cooperation and defection with common-interest in the IPD becomes the mean return of both agents, formally $\mathbb{E}(C) = \frac{2(b-c)}{2} + \frac{b-c}{2}$ and $\mathbb{E}(D) = \frac{b-c}{2}$.
Without knowing opponent strategies, this means the expected values of cooperation and defection with common interest in the IPD becomes the mean return of both agents, formally $\mathbb{E}(C) = \frac{3(b-c)}{2}$ and $\mathbb{E}(D) = \frac{b-c}{2}$.
Since $b > c$ is required, $\mathbb{E}(C) - \mathbb{E}(D) = b - c$, making (C, C) the unique Nash Equilibrium and Pareto Efficient strategy.
% The common-interest scenario makes $\mathbb{E}(C) > \mathbb{E}(D)$ and the Nash Equilibrium and only Pareto Efficient strategy (C, C).
This changes the dynamics of the IPD where (D, D) is the unique Nash Equilibrium and (C, C), (C, D), and (D, C) are the three Pareto Efficient strategies.


From the view of $T_i$, our model of teams preserves mixed-motive interactions with agents on other teams, but transforms interactions with agents in $T_{i}$ to be common interest.
Using the frequencies of interacting with agents in $T_{i}$ ($\inteam$) and other teams ($\outteam$), we calculate the expected value of cooperation and defection with teams by Equations \ref{eq:team_coop} and \ref{eq:team_def}.

% \begin{equation}
%     \mathbb{E}(C)_{\mathcal{T}} = \left(\frac{b-2c}{2}\right)\overline{t} + \left(\frac{2(b-c)}{2} + \frac{b-c}{2}\right) t
%     \label{eq:team_coop}
% \end{equation}

\begin{equation}
    \mathbb{E}(C)_{\mathcal{T}} = \left(\frac{b-2c}{2}\right)\outteam + \left(\frac{3(b-c)}{2}\right) \inteam
    \label{eq:team_coop}
\end{equation}

\begin{equation}
    \mathbb{E}(D)_{\mathcal{T}} = \left(\frac{b}{2}\right)\outteam + \left(\frac{b-c}{2}\right) \inteam
    \label{eq:team_def}
\end{equation}

Since we are unaware of the prior distribution of opponent strategies, the expected value of either action becomes dependent on how often an agent interacts with their teammates $\inteam$ and non-teammates $\outteam$.
We derive the lower bound scenario where the common interest Nash Equilibrium and Pareto Efficient strategy are preserved despite mixed-motives between teams.

\begin{equation*}
    \mathbb{E}(C)_{\mathcal{T}} = \mathbb{E}(D)_{\mathcal{T}}
\end{equation*}

% \begin{equation*}
%     \left(\frac{b-2c}{2}\right)\overline{t} + \left(\frac{2(b-c)}{2} + \frac{b-c}{2}\right) t = \left(\frac{b}{2}\right)\overline{t} + \left(\frac{b-c}{2}\right) t
% \end{equation*}

\begin{equation*}
    \left(\frac{b-2c}{2}\right)\outteam + \left(\frac{3(b-c)}{2}\right) \inteam = \left(\frac{b}{2}\right)\outteam + \left(\frac{b-c}{2}\right) \inteam
\end{equation*}

\begin{equation*}
    \left(\frac{b-2c}{2}\right)\outteam + \left(\frac{2(b-c)}{2}\right) \inteam = \left(\frac{b}{2}\right)\outteam
\end{equation*}

\begin{equation*}
    -c\outteam + b\inteam - c\inteam = 0
\end{equation*}

\begin{equation*}
    -c (\outteam + \inteam) + b\inteam = 0
\end{equation*}

\begin{equation}
    b\inteam > c
    \label{eq:equilibrium}
\end{equation}

Recall that $\inteam \leq 1$ is the frequency of interactions $i$ has within their own team $T_{i}$.
The derivation results in Equation \ref{eq:equilibrium}, meaning that $b\inteam > c$ is required to preserve the IPD game-theoretical properties of the common interest scenario in expectation.
When $b\inteam \leq c$, the game-theoretical properties are consistent with the regular IPD.

% \todo{Maybe talk about how teams transform into a collective risk dilemma? Full equilibria is transforming IPD into CRD and defecting up to $\tau$ amount against other teams.}


\end{comment}

==> ethics.tex <==

\section{Ethics Statement}

% \todo{This can be on reference page. ``An ethics statement that addresses both ethical issues regarding the research being reported, and the broader ethical impact of the work."}



% \todo{Maybe move to ethics statement as a side-effect.}
% When constructing teams in practice, our evaluation shows the importance of being cognisant of potential side-effects of some team structures given some environments.
% In Cleanup, we find that 3/2 achieves the highest reward at the cost of less equality due to a free-riding team.
% Therefore, one might consider the 2/3 team structure to be a more stable result considering the high reward and higher equality with the default Cleanup environment dynamics.


% \todo{Could move below to ethics statement.}
% However, $T_{1}$ (red) in the 3/2 scenario ends up free-riding on the labor of other teams to support the four apple picker joint policy which leads to less equality in Figure~\ref{fig:cleanup_equality}.
% Note that the other two teams continue to clean the river and the efficient joint policy remains stable despite the free-riding team.

% It is important to consider how the side effects of certain team structures may result in slight inequalities among agents.
While our 3/2 team structure achieves high reward in Cleanup, it has higher inequality than 2/3.
This is a side effect the best joint policy in Cleanup being four apple pickers and two river cleaners.
For 3/2 to achieve this division of labor, one team ($T_{1}$ (red) in Figure~\ref{fig:div_labor}) must free-ride on the labor of the other two teams.
% Despite the resulting inequality, the other two teams continue to clean the river and the environment remains stable; however, this stability could be reliant on a surplus of apples.
Systems should account for these potential side effects if slight inequality is detrimental to its welfare in the long-run despite short-term stability.
% Therefore, one might consider an alternate team structure, such as one with both high reward and equality (i.e., 2/3), when defining teams depending on the overall goal of the system.

% \clearpage
% \newpage

%%%KATE: This will help with getting the spacing right in the 6 page part of the paper.


==> preliminaries.tex <==
% \todo{This will be $\frac{1}{2}$ column.}

% Presents syntax and notation.
% It will also define what ``decentralized" vs. ``centralized" policies are, and ``selfish" vs. ``system"-oriented behavior.
% These will be aligned with mixed-motive and common-interest terms as well.


We are interested in settings where agents have repeated interactions and are unable to explicitly modify their social network.
% , such as repeated two-player matrix games between \emph{any} two agents in a population.
Our environment is modeled as a stochastic game represented by the tuple: $\langle N, \mathbf{T}, S, A, \mathbf{R}, \Sigma \rangle$.

$N$ represents the set of all agents in a population.
A \emph{team} is a subset of $n \subset N$ agents and $i$ is any arbitrary agent.
$\mathbf{T} \geq 2$ is the set of all teams in the system,
agent $i$ belongs to team $\mathbf{t}_{i}$, and the set of all remaining teams is denoted $\mathbf{T}^{-\mathbf{t}_{i}}$.
% The set of teams $\mathbf{T}$ is indexed as $\{\mathbf{t}_{1}, \dots, \mathbf{t}_{i}, \dots, \mathbf{t}_{|\mathbf{T}|}\}$, where $|\mathbf{T}| \geq 2$, $i \in \mathbf{t}_{i}$ and $\mathbf{T}^{-\mathbf{t}_{i}}$ represents all other teams besides $\mathbf{t}_{i}$.
$S$ represents the joint state space of all agents in $N$, defined as $S_{\mathbf{t}_{i}} = \{S_{1}, \dots, S_{i}, \dots, S_{n}\}$ for a single team.
$A$ represents the joint action space of all agents, and $A_{\mathbf{t}_{i}} = \{A_{1}, \dots, A_{i}, \dots, A_{n}\}$ represents the joint action space of team $\mathbf{t}_{i}$.
$R$ represents the joint reward function of all agents, and a team $\mathbf{t}_{i}$ has joint reward function $\mathbf{R}_{\mathbf{t}_{i}} = \{ R_{1}, \dots, R_{i}, \dots, R_{n} \}$, where $R_{i} : A_{i} \rightarrow \mathbb{R}$ is the reward function for agent $i \in \mathbf{t}_{i}$ which returns a real-numbered rewards for taking actions.
A single reward obtained by agent $i$ is denoted $r_{i} \in R_{i}$.
The joint policy of all agents is $\Sigma$, however $\Sigma_{\mathbf{t}_{i}} = \{\pi_{1}, \dots, \pi_{i}, \dots, \pi_{n}\}$ represents the joint policy of team $\mathbf{t}_{i}$, where $\pi_{i}$ is the policy of agent $i$.


Our analysis uses the IPD two-player matrix game which models an interaction between two agents.
For the sake of modeling these interactions, we label a focal agent $f$ and their opponent $o$.
Throughout the paper, we use the notation of $i$, $f$, and $o$ to refer to agents depending on the situation.
In each episode, or round of interactions, all $N$ agents are $f$ exactly once.
Agent $f$ randomly samples an opponent $o$ from the remaining $N-1$ agents, unable to choose with themselves.
$f$ and $o$ choose an action simultaneously and each receive $r_{f}$ or $r_{o}$ respectively without viewing each other's action.
Note that in any episode, an agent $i$ will be $f$ in one interaction and could be chosen by another agent to be $o$, meaning agents could have anywhere between $1$ and $N$ interactions each episode.
In this case, $r_{i}$ is the mean reward obtained by $i$ for that episode.
% Social welfare is a traditional metric in mechanism design and MAS, defined as the mean of player utilities achieved by all players.



==> rogue_intro.tex <==

\section{Unreliable Agents}


A team is usually most productive when all agents are capable and construct similar models of their goals; however, this may not always be the case.
Sometimes \emph{unreliable} agents exist who, for whatever reason, are unable to perform tasks as expected.
In the context of our two social dilemmas, unreliability can mean various different things since the dynamics of the IPD and Cleanup are extremely different.
For clarity, we define unreliability specifically for the IPD and Cleanup and represent the set of unreliable agents on team $T_i$ as $\mathbf{x}_{T_i}$.

% \begin{definition}
%     A \emph{rogue agent} $x \in 
%     T_i$ is an agent that may or may not take the action that is defined by their policy with some probability $d$ at every timestep.
%     The set of rogue agents on team $T_i$ is denoted $\mathbf{x}_{T_i}$.
% \end{definition}

% In our experiments, we define $d$ as the \emph{degree of rogueness} which is set \emph{a priori} to be the same for all rogue agents, though this is not a requirement.

\noindent
\textbf{IPD: }
An unreliable agent in the IPD is one that chooses defection with some probability $d$ at each timestep.
Evolutionary mean field theory shows how an initially small amount of defecting agents will ultimately steer the population to defection~\cite{Sigmund2010TheCO}.
In Appendix C, we prove how team size mitigates the negative spread of unreliable agents and sustains cooperation as the dominant action.
Our empirical evaluation with MARL agents confirms our derived theory in the context of the IPD.



% \begin{definition}
%     %Rogue Agent \\
%     A \emph{rogue agent} $x \in 
%     T_i$ in the IPD is an agent that cooperates some amount less than their equal share of the group, $\frac{C^{T_i}_{T_j}}{|T_i|} - \epsilon$.
%     The set of rogue agents on team $T_i$ is denoted $\mathbf{x}_{T_i}$.
%     % \Kate{You have a notation problem. $C_{T_j}^x$ is referring to a single agent $x$ while you are also using $C_{T_j}^{T_i}$ to mean the team $T_i$. This is confusing since $x$ is part of $T_i$. Can you use something else? Like I don't even know why you need the fraction.}
% \end{definition}

% In the context of social dilemma domains where agents are unable to choose their social graph,
% the model of the IPD studied here, where all agents have equal probability of interacting, 
% Evolutionary mean field theory shows how an initially small amount of defecting agents will ultimately steer the population to defection~\cite{Sigmund2010TheCO}.
% In Appendix C, we prove how team size mitigates the negative spread of rogue agents using the definition above.


\noindent
\textbf{Cleanup: }
The action space in Cleanup is more complex than the IPD, thus we define an unreliable agent in Cleanup as one that chooses a random action with some probability $d$ at each timestep.

% \begin{definition}
%     %Rogue Agent \\
%     A \emph{rogue agent} $x \in 
%     T_i$ in Cleanup is an agent that acts randomly with some probability at each timestep.
%     The set of rogue agents on team $T_i$ is denoted $\mathbf{x}_{T_i}$.
% \end{definition}





% While rogue agents threaten team and system success, we show how team structures mitigate the negative impact of rogue agents and allow for sustained cooperation in the population.
% % the size of teams mitigate the impact they have.
% \newtext{
% Since cooperation and defection are not explicit actions agents can take in Cleanup, we simply define a rogue agent in Cleanup as one that acts randomly given some probability.
% }




% \subsubsection{Number of Teams and Global Return}

% This analysis shows how the number of teams $|\mathbf{T}|$ impacts global return in the presence of rogue agents.
% Specifically, consider a situation where $\mathbf{x}$ affects their team reputation enough to prevent mutual cooperation with other teams.
% We identify that as $|\mathbf{T}|$ increases, the negative impact of rogue agents on global return decreases.


% \begin{theorem}
% The negative impact of rogue agents $\mathbf{x}$ on global return decreases as $|\mathbf{T}| \rightarrow \infty$, the number of teams increases.
% \label{thm:team_amount_inc}
% \end{theorem}

% \begin{proof}
% Assume our model of teams.
% % , however non-rogue agents are never able to cooperate enough to sustain $C^{\mathbf{t}_{f}}_{\mathbf{t}_{o}} > \tau$.
% Our framework requires $|\mathbf{T}| \geq 2$, $n \geq 1$, $|\mathbf{t}_{f}| = |\mathbf{t}_{o}|$, and $\mathbf{x}_{\mathbf{t}_{f}} < n$ when $n > 1$.
% Therefore, the two extremes for number of teams are: $|\mathbf{T}| = 2$ where $n = \frac{N}{2}$ and $|\mathbf{T}| = N$ where $n = 1$.

% When $|\mathbf{T}| = 2$, suppose there exists $\mathbf{x} < \frac{N}{2}$ rogue agents all on one team that prevents the frequency of cooperation from reaching $\tau$.
% % and prevent $C^{\mathbf{t}_{i}}_{\mathbf{t}_{j}} > \tau$.
% The reputation of all $\frac{N}{2}$ agents on this team will be negatively impacted, meaning both teams will defect and reward will be low.
% Since $|\mathbf{x}| < n$, we know there exists at least one non-rogue agent on this team that is negatively impacted by poor reputation.

% % This includes the $n - |\mathbf{x}_{\mathbf{t}_{f}}|$ non-rogue agents on $\mathbf{t}_{f}$.
% When the number of teams grows and $|\mathbf{T}| = N$, only the reputations of $\mathbf{x}$ agents will be impacted, and the reputation of the remaining $N - |\mathbf{x}|$ agents will depend on their non-rogue behavior.
% Therefore, $N - |\mathbf{x}| > \frac{N}{2}$ agents in the second case are able to mutually cooperate and increase global return, whereas only $\frac{N}{2}$ could in the first case with fewer teams.
% % Thus, the negative impacts will only be limited to agents in $\mathbf{x}_{\mathbf{t}_{i}}$ meaning more agents will be able to cooperate and global welfare will increase.
% \end{proof}

% Intuitively, the negative impact of rogue agents will be less detrimental to global return as they impact the reputation of fewer non-rogue agents.
% Since cooperation achieves the highest global return, Theorem \ref{thm:team_amount_inc} shows how more agents are able to cooperate as the number of teams increases and rogue agents become more isolated.



==> rogue_results.tex <==

\subsection{Unreliable Agents Evaluation}
%\todo{Is it okay to have two subsections titled ``Rogue Agents"?}
%\Kate{Nope -- need to re-organize your subsection titles -- in particular you should have two subsections under the "Rogue Agent" heading}.

In our next set of experiments we explore whether team structures are robust to the impacts of unreliable agents.
% Recall that an unreliable agent is one that is unreliable so that, for whatever reason, it will choose defection some of the time.  
We evaluate different team structures for various amounts of unreliability and investigate the number and size of teams.
We use the same team compositions as the previous experiments and
%meaning when $|\mathcal{T}| \geq 5$ the game-theoretical properties favor %defection by Equation \ref{eq:equilibrium}.
define a \emph{degree of unreliability} $d \in [0,1]$.
% so that $a_i = D$ with probability $d$ and $a_i$ comes from $\pi_i$ with probability $1-d$.
% rogue agents choose defection with probability $d$. 
We experiment with $d\in\{0.25, 0.5, 0.75\}$. 
We assign unreliable agents to teams so that $|T|-1$ unreliable agents are assigned to $T_0$ (Team 0) before any are assigned to $T_{1}$, etc. 
This was done to help analyze how agents react to teams with various proportions of unreliable agents. 
Specifically, we want to understand if agents can learn to distinguish teams with a higher fraction of unreliable agents from teams without unreliable agents.
We show results for games where $c=1$ and $b=5$ since these values showed team structures encourage cooperation despite the incentive to defect when $|\mathcal{T}| \geq 5$.
%\todo{Other findings or other work? When $b=2$, the results are very different since agents only cooperate with their teammates. Other work does use $c = 1$ and $b = 5$ though.}
%\newtext{Maybe: We show results for games where $c=1$ and $b=5$ to be consistent with past work and since agents originally learned to solve the social dilemma in this case.}


\subsubsection{Unreliable Agents and Number of Teams}

% \Kate{Clean up this paragraph so that it does not repeat anything that is listed above. Make sure the rest is very clear. Like what is $x$? Do you need to mention it here? I still don't understand why you have unbalanced rogue agents here -- ie some teams will have no rogues while others will be completely rogue. You should justify this choice. }
% Next, we analyze how the number of teams in a fixed population impacts the affect of rogue agents.


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/heatmap_return_gini-star-all7.png}
    % \vspace{-10pt}
    \caption{Impact of unreliable agents with various team compositions when $c = 1$, $b = 5$, and the degree of unreliability changes $d \in \{0.25, 0.5, 0.75 \}$. We record a) average global reward and b) Gini index where red is better, and indicate the row with the highest average and lowest Gini index (not considering confidence intervals) with a star.}
    \label{fig:exp-grid_all}
\end{figure}

% We experiment with different amounts of rogue agents and three different degrees of rogueness, so $d \in \{0.25, 0.5, 0.75\}$.
Figure \ref{fig:exp-grid_all}a shows the average global reward obtained for various values of $d$ with increasing numbers of unreliable agents.
Individual plots show the number of unreliable agents in the population along the $y$-axis and the team compositions along the $x$-axis.
The team composition that achieves the highest reward for each number of unreliable agents (each row) is labelled with a star.
% Each square represents a different simulation with the parameters along either axis.
Our results show that more teams generally improve the reward as the number of unreliable agents increases, consistent for all values of $d$.
However, note that when $|\mathcal{T}|\geq 5$, the overall gain in average return is small. 
Thus, if there is overhead required to create and maintain team structures, fewer teams could be considered even if there are concerns about unreliable agents.
%We also find that there are marginal reward gains, if any, when $|\mathcal{T}| \geq 5$ meaning creating more teams may not be desired if the cost of forming teams is high.


Average reward does not fully capture the entire picture of how teams perform. 
Fairness in reward is also of interest. 
The Gini index is a measure of how equitably a resource is distributed in a population, commonly used in economics~\cite{Ceriani2012TheOO}.
The index is the mean difference from all quantities, so lower values represent more equality.
Given $\overline{R_{N}}$ as the mean population reward, the Gini index is calculated by:

\begin{equation}
    Gini = \frac{\sum_{i=0}^{N} \sum_{j=0}^{N} |R_i - R_j|}{2|N|^{2} \overline{R_{N}}}
\end{equation}


% \Kate{IS there a formula you can add here? You want to be as precise as possible so someone else can redo your results}.
Figure \ref{fig:exp-grid_all}b shows the Gini index of the population with the same values of $d$ and axes.
% \Kate{Formally define the Gini index!! Like how did you compute it? Provide a citation? This is a standard measurement but not everyone is going to know it}
% Gini index is a measure of inequality common in economics where lower values suggest a more equal population.
We reverse the color scheme so red still indicates a better result (i.e., more equality) and use a star to indicate the most equal team composition for each number of unreliable agents omitting confidence intervals.
Our results show fewer teams of more agents typically leads to high inequality since unreliable agents impact more of the population. %non-rogue teammates than when teams are small.
As the population is configured into more teams, the Gini index decreases and the population has more equality.
%Depending on $d$, we again see marginal gains in equality when $|\mathcal{T}| \geq 5$ in this setting.
% \Kate{I Do not understand this last sentence -- maybe just cut it}
% Given $d$ and a number of rogue agents, pairing average reward and Gini index together could provide insight into a desirable team composition.
% For most amounts of rogue agents, we find that 3, 5, and 6 teams generally have the most equality.
% Figure \ref{fig:exp-more-teams}a and b together show how more teams generally mitigate the negative impacts of rogue agents, allowing for higher global reward and more equality.
% This is consistent our derived theory on the impact of multiple interdependent teams to mitigate incompetent agents.






%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


% below is 3rd experiment without coop

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/heatmap_teams_grow_nonorm-full2.png}
    % \vspace{-10pt}
    \caption{unreliable agents and growing team size with $|\mathcal{T}| = 3$ and $d = 0.5$. We record the difference in average a) $Q$-values of cooperation when matched with $T_{0}$ and b) reward of $T_0$ compared with the average of $T_1$ and $T_2$.}
    \label{fig:team_size}
\end{figure}


\subsubsection{Unreliable Agents and Size of Teams}

Theorem \ref{thm:team_size_increase} in the appendix suggests that the negative impact of unreliable agents on the perceived value of cooperating with $T_i$ decreases as the team size ($|T_i|$) increases.
To isolate the effect of $|T_i|$, we keep the state space consistent so $|\mathcal{T}| = 3$ and set $d = 0.5$, but modify the size of teams so $|T| = 4,6,8,10$, thus increasing the size of the agent population.
We experiment with one, two, and three unreliable agents on Team 0 ($T_{0}$).
% We analyze two characteristics: the perceived value of cooperating with $T_{0}$ and the average reward obtained by $T_{0}$ relative to the other teams.
\begin{comment}
\Kate{ OK -- I see what you are doing -- I got very confused. Cut the rest of this paragraph. Then have one paragraph that **only** talks about Figure 3a and. Then have a second paragraph that only talks about Figure 3b.}
We analyze two metrics in this set of experiments by comparing $T_0$ which has rogue agents to $T_1$ and $T_2$.
First, we compare how agents perceive the value of choosing cooperation when paired with $T_0$ with when they are paired with the other teams.
% with the mean of the other two teams.\Kate{What do you mean by "Mean of the other two teams". Mean of what}
Next, we calculate the difference between the average reward obtained by $T_0$ and the mean reward of the other teams.
\end{comment}
% \Kate{ I Do not understand what this sentence means. Cut it: The values $c = 1$, $b = 5$, $\alpha = 1$, $|\mathcal{T}| = 3$ suggest cooperative game theoretic properties in this setting, however the RL agents learn alternative behavior in different scenarios.}

In our first experiment we are interested in understanding if agents perceive cooperation differently with teams $T_1$ and $T_2$ than with $T_0$ which has unreliable members.
We do this by comparing the $Q$-values of agents, their learned expected value, for the cooperation action when they are paired with $T_0$ to when they are paired with agents from either $T_1$ or $T_2$. 
We omit the $Q$-values of unreliable agents since, by design, we interfere with their policies.
%To estimate the perceived value of choosing cooperation, we average the Q-values for cooperation when agents are paired with teams other than their own.
%Since we directly alter the actions taken by rogue agents, and therefore how they learn, we omit their Q-values.
% The Q-value for cooperation given a team label describes agents' expected value of cooperating, consistent with our definition.
% We analyze the Q values of each agent which represent their beliefs of the value for taking an action.
% In this case we aggregate the Q value for choosing C against each team from agents not on that team and calculate the difference from $T_{0}$ to the other teams.
Figure \ref{fig:team_size}a shows the difference between the average $Q$-values when agents are paired with $T_0$ and when they are paired with $T_1$ and $T_2$.
% \Kate{CAn  you reword the previous sentence to make it more clear. I find it a little hard to understand}
The $y$-axis shows the size of each team and the $x$-axis shows number of unreliable agents in $T_{0}$.
A difference of zero (white) means agents expect the same value when cooperating with $T_0$ as they do with $T_1$ and $T_2$, and negative (blue) means they expect less value.
% Negative (blue) means agents expect less value when cooperating with $T_0$ than when cooperating with the other teams.
% the Q-values are less than the mean of cooperating with the other teams.\Kate{ What does the previous sentence mean. I do not understand what you mean by Q-values are less than the mean of cooperating....}
Figure \ref{fig:team_size}a shows that agents value cooperation with $T_0$ less than with the other teams in all settings.
However, this impact is decreased with fewer unreliable agents and as $|T|$ increases, which is consistent with Theorem \ref{thm:team_size_increase}.


%We now compare the average reward obtained to further analyze the impact of rogue agents on team performance.
% \Kate{ Can you rewrite this? I am having trouble following what you want to say.}
Figure \ref{fig:team_size}b compares the average reward obtained by $T_{0}$ to the average reward of the other two teams $T_1$ and $T_2$.
We use the same axes as before, where zero (white) means $T_0$ achieves the same reward as the other teams.
% We show the size of each team $|T|$ along the y-axis and the number of rogue agents on $T_{0}$ $|\mathbf{x}_{T_{0}}|$ along the x-axis.
When $T_0$ has one unreliable agent, $T_{0}$ achieves more reward than the other teams.
This is caused by agents on other teams cooperating with $T_0$ when the unreliable agent chose defection and received the full benefit.
% These gains are mitigated as $|T|$ increases since more non-rogue agents decreases the mean reward obtained by the one rogue agent. 
% \todo{Should I divide by $|T|$ in each row for mean reward difference?}
When $T_{0}$ has two unreliable agents, we observe instances where $T_0$ achieves more or less reward than the other teams,
%the other teams sometimes learn to defect on $T_0$ and sometimes do not, 
likely due to the stochastic learning process of the agents.
% Regardless of the learned behavior, the difference decrease as $|T|$ increases.
When $T_{0}$ has three unreliable agents, teams learn to defect on $T_0$ when $|T| < 10$, and $T_1$ and $T_2$ cooperate with amongst themselves which increases their average reward relative to $T_0$.
% and causes $T_0$ to achieve less relative reward.
% This causes $T_0$ to achieve less reward relative to the other teams.
However when $|T| = 10$, $T_{0}$ achieves basically equal reward despite three unreliable agents.

% \todo{Should I cut this paragraph? I figured it might be good to explain why Q-values for cooperating with $T_0$ are worse (blue) in Figure \ref{fig:team_size}a but the team does better in Figure \ref{fig:team_size}b. It might be confusing to revisit after the previous paragraph though.}
% \Kate{I think it is an interesting point BUT can you condense it?}
Note that when $|T_0| < 10$ with one unreliable agent, $T_0$ achieves more reward than the other teams despite agents expecting cooperation with $T_0$ to be less valuable than with other teams.
This is caused by agents still valuing cooperation with $T_0$ more than defection, so the slight defection from $T_0$ collects more reward but is not frequent enough to change the policies of agents towards defection.
% The slight defection by the rogue agent on $T_0$ collected more reward over time but was not frequent enough to cause agents to learn defection.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 

% below is 3rd experiment WITH coop figure

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth]{Figures/heatmap_return_coop_rep.png}
%     % \vspace{-10pt}
%     \caption{Impact of rogue agents and $n$ with a consistent state space of $|\mathbf{T}| = 3$. We record the a) difference in average reward, b) percent of cooperation from Team 0, and c) difference in Q values for $\mathbf{t}_{0}$ compared to $\mathbf{T}^{-\mathbf{t}_{0}}$.}
%     \label{fig:team_size}
% \end{figure}


% \subsubsection{Rogue Agents and Size of Teams}
% Theorem \ref{thm:team_size_increase} suggests that the negative affect of rogue agents on team reputation decreases as $n$, the size of the team, increases.
% To isolate the affect of $n$, we now keep the state space consistent so $|\mathbf{T}| = 3$ and increment $n \in (4,10)$.
% We experiment with 1, 2, and 3 rogue agents on Team 0 ($\mathbf{t}_{0}$), and analyze the performance of $\mathbf{t}_{0}$ relative to $\mathbf{T}^{-\mathbf{t}_{0}}$.
% The same values for $c$, $b$, and $\alpha$ as before with $|\mathbf{T}| = 3$ suggest cooperative game theoretic properties in this setting, however the RL agents respond differently when there are more rogue agents in $\mathbf{t}_{0}$.


% Figure \ref{fig:team_size}a shows the difference in average reward from $\mathbf{t}_{0}$ compared with $\mathbf{T}^{-\mathbf{t}_{0}}$, where zero (white) means they have equal reward, and Figure \ref{fig:team_size}b shows the percent of cooperation from $\mathbf{t}_{0}$ to analyze what $\tau$ actually is with RL agents.
% We show the size of the team $n$ along the y-axis and the number of rogue agents $|\mathbf{x}_{\mathbf{t}_{0}}|$ along the x-axis.
% In the first column of Figure \ref{fig:team_size}a and b with 1 rogue agent, opponents do not learn to defect and the cooperation percentage from $\mathbf{t}_{0}$ is high, achieving higher reward than the average.
% These gains are mitigated as $n$ increases and mutual cooperation becomes more standard.
% In the second column when $\mathbf{t}_{0}$ has 2 rogue agents, we observe mixed instances when opponents learn to defect against $\mathbf{t}_{0}$, however these affects are mitigated as $n$ increases seen by lighter shades of color.
% The cooperation percentage of $\mathbf{t}_{0}$ is lower, seen by comparing columns 1 and 2 of Figure \ref{fig:team_size}b, however it seems as though $\tau$ changes slightly depending on $n$.
% The third column shows when $\mathbf{t}_{0}$ has 3 rogue agents and opponents clearly learn defection when $n$ is small, seen through the low comparative reward for $\mathbf{t}_{0}$.
% This low reward is mitigated as $n$ increases and $\mathbf{t}_{0}$ achieves about the same reward as the other teams when $n = 10$ despite having 3 rogue agents.
% Pairing this result with the low cooperation percentage from $\mathbf{t}_{0}$ in the third column of Figure \ref{fig:team_size}b shows how $\mathbf{t}_{0}$ fails to solve the CRD which leads to other teams learning defection.

% Our second analysis aims to directly analyze the aspect of Theorem \ref{thm:team_size_increase} about the impact of rogue agents on team reputation as $n$ increases.
% We analyze the Q values of each agent which represent their beliefs of the value for taking an action.
% In this case we aggregate the Q value for choosing C against each team from agents not on that team and calculate the difference from $\mathbf{t}_{0}$ to $\mathbf{T}^{-\mathbf{t}_{0}}$.
% Figure \ref{fig:team_size}c shows our results for the difference in Q value for C where zero (white) means they are equal and negative (blue) means the Q value is less than the mean.
% All regions being blue suggests the reputation of $\mathbf{t}_{0}$ is always negatively impacted by rogue agents, however the lighter shades mean reputation is generally less affected with higher value of $n$ and fewer rogue agents.
% This finding empirically confirms Theorem \ref{thm:team_size_increase} in our model of teams, showing that agents expect playing C to have less value against $\mathbf{t}_{0}$ than against teams without rogue agents, $\mathbf{T}^{-\mathbf{t}_{0}}$, but this impact decreases as $n$ increases.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 


















% This section tests the framework empirically.

% \begin{itemize}
%     \item Experiment to show cooperation is learned using MARL agents with decentralized policies.
    
%     \item Compare with fully selfish and system oriented IPD. What is the advantage here over system oriented? (cant always have system oriented agents in the real world, do not always have control).
%     Analyze ratio of mutual cooperation, temptation, sucker, and mutual defection in experience (show that there is more cooperation compared to selfish)
    
%     \item \newtext{4 experiments: } Perform studies to confirm 1) as team size increases, agents play roughly the same number of games, 2) negative impact of incompetent agent decreases with population size, 3) as number of teams grow, impact of incompetent agent on global welfare decreases, 4) equilibrium analysis, modify $t$ and see how cooperation emerges with teams despite non-cooperative game characteristics.
% \end{itemize}



% FIRST: 

% show teams lead to cooperation:
% -compare 30 teams/1 agent - 5 teams/6 agents - 1 team/30 agents for c:b (normal, team, cooperative) for cooperation \% and reward
% -equilibrium analysis, teams sustain cooperation given THIS far of a stretch into uncooperative game properties

% INCOMPETENT AGENTS:
% maybe:
% add chart showing as team size/population grows, cooperation/reward increases

% definitely:
% show the 2, 3, 5, 6, 10, 15 team chart with growing inc agents
%     -could analyze reward, cooperation, gini index?





Here are my results for the cleanup environment.

==> social_dilemmas.tex <==
% \todo{This will be $\frac{1}{2}$ column.}

% Discusses social dilemmas and the iterated prisoner's dilemma.

For normal-form matrix games studied in game theory, the behavior of an agent can be generally thought of in the context of ``cooperation" (C) and ``defection" (D).
% In Game Theory, the behavior of a rational agent can be generally thought of in the context of ``cooperation" (C) and ``defection" (D).
A \emph{social dilemma} is a situation in which each individual receives a higher payoff for defecting than cooperating, but all are better off if all cooperate than if all defect~\cite{Kendall2018TheCO,dawes2000}.
The failure to solve social dilemmas comes from acting in a way which seems individually rational, however this leads to agents being worse off than if they acted irrationally.
% The failure to solve social dilemmas and support extensive cooperation is caused by selfish behavior since the payoff of defecting is higher than cooperating unless everyone chooses to defect~\cite{Dawes1980SocDilemmas}.
Real-world social dilemmas include resource depletion~\cite{Brady1993GoverningTC}, donating money~\cite{dawes2000}, and wildfire fuel mitigation~\cite{Norton2020ComputingDefensibility}.
These are classified as ``mixed-motive problems" and are difficult for rational RL agents to solve, or cooperate, without additional infrastructure~\cite{Kraus1997NegotiationAC}.
Studying situations in which rational agents overcome the short-term incentive to defect to experience long-term benefits is of growing interest in artificial intelligence (AI).


\begin{table}
\begin{center}
 \begin{tabular}{|c||c|c|} 
 \hline
  & Cooperate & Defect \\ [0.5ex] 
 \hline\hline
Cooperate & $b-c$ $\setminus$ $b-c$ & $-c$ $\setminus$ $b$ \\\hline
Defect & $b$ $\setminus$ $-c$ & $0$ $\setminus$ $0$ \\
 \hline
\end{tabular}
\caption{Special case Prisoner's Dilemma with the costs (c) and benefits (b) of cooperating.}
\label{tab:pd_table}
\end{center}
\end{table}

One of the most well studied social dilemmas is a two-player (row, column) normal-form matrix game called the Prisoner's Dilemma (PD).
Table \ref{tab:pd_table} shows a special version of the PD that we use in our analysis which uses the costs (c) and benefits (b) of cooperating to calculate payoffs, where $b > c$ required.
If both players choose to cooperate, they both pay the cost of cooperation and both receive the benefit.
If only one cooperates, the defector receives the benefit leaving the cooperator to pay the cost, but both defecting causes neither to pay the cost nor receive any benefit.
When agents repeatedly play the PD it is known as the Iterated Prisoner's Dilemma (IPD).
Since the opponent's strategy is unknown prior to the game, the expected values of cooperating $\mathbb{E}(C)$ and defecting $\mathbb{E}(D)$ are calculated as the mean return of each action, shown in Equations \ref{eq:exp_c} and \ref{eq:exp_d}.


\begin{equation}
    \mathbb{E}(C) = \frac{b-2c}{2}
    \label{eq:exp_c}
\end{equation}

\begin{equation}
    \mathbb{E}(D) = \frac{b}{2}
    \label{eq:exp_d}
\end{equation}


The joint strategy which leads to the highest global return is if both cooperate (C, C).
However, the unique Nash Equilibrium, defined as when no agent has incentive to deviate from their strategy and achieve higher payoff, of the finitely-repeated IPD is to always defect (D, D).
The Pareto Efficient strategies, where no agent can improve their strategy without negatively impacting another agent's payoffs, of the game are (C, C), (C, D), and (D, C).
From the utilitarian idea of maximizing the number of agents who achieve high payoffs, Pareto Efficient outcomes are desirable.

% \todo{Add something here about collective risk dilemmas.}

\subsubsection{Collective Risk Dilemma}

% There exists social dilemmas beyond the framework of two-agent normal-form games, most notably the collective risk dilemma (CRD).
% The CRD 

Beyond two-player games, a collective risk dilemma (CRD) is a type of social dilemma with non-linear payoffs among a population of more than two agents.
The CRD is also called the threshold Public Goods Game (PGG), where agents need to merge their individual efforts to achieve a certain cost threshold and avoid a common risk.
Real world examples of a CRD include action against climate change or receiving a vaccine for COVID-19.
Agents must individually decide whether to pay the cost of cooperation, but if the total cost paid by the group fails to reach a defined threshold, every agent experiences the disaster regardless if they paid the cost.

In our work, we find that our model of teams playing repeated two-player games such as the IPD causes a CRD to emerge within each team, a second-order social dilemma.
Specifically, a team has the best collective payoffs when they all play D and their opponents play C, however repeatedly playing D against opponents will cause them to eventually also play D and converge to the Nash Equilibrium.
The CRD emerges when teams must learn to collectively cooperate with opponents enough to avoid them learning to play D, but then playing the occasional D to collect higher payoffs in the long run.
In this case, a new Nash Equilibrium emerges if all teams follow this strategy simultaneously.

==> teams_model.tex <==
\section{Model of Multiagent Teams}
\label{sec:teams_model}

% \todo{This will be 1 column}

% Introduce model of teams, how shared their focus is, is there communication, etc...

\Kate{Things to think about: What is specific to your actual testbed and what is more generic? Bring anything that is generic into the earlier section. Push everything that is very specific into an implementation details section. A good example is the stuff about one-hot vector in structure and observability. That is implementation stuff -- not part of the model}


% Our model of teams is not directly related to the work in Team Forming, where the goal is to cover a set of requirements while optimizing for robustness and efficiency~\cite{Schwind2021PartialRI,Shah2020BenefitsOA}.
% skill of a team is the union of all member agents and performance is based on task coverage, robustness to errors, and efficiency~\cite{Schwind2021PartialRI,Shah2020BenefitsOA}.
Instead of trying to find the \emph{best} teams from a set of agents as done in Team Forming and CSG, we design a team structure of MARL agents to impact online learning.

\subsection{Structure and Observability}
% We denote the team containing agent $i$ as $\mathbf{t}_{i} \in \mathbf{T}$, and all other teams as $\mathbf{T}^{-\mathbf{t}_{i}}$.
However similar to Team Forming, we impose restrictions on the composition of teams.
First, we restrict teams to have the same number of agents, $|\mathbf{t}_{f}| = |\mathbf{t}_{o}| = n \forall f, o \in N$, where $n > 1$.\Kate{Does this matter in general? Or is this an implementation detail here? It certainly limits the generality of your model...}
We assume a complete social graph so any agent could interact with any other agent in the population except for themselves.
% An ``interaction" defines one play of the IPD game between two agents, $f$ and $o$.
% In our environment, an agent $f$ chooses an opponent $o$ from the remaining $N - 1$ agents and plays one iteration of the Prisoner's Dilemma game, which we call an ``interaction".
When playing the IPD, we also assume incomplete information and partial observability by $f$ only observing the team label for $o$, and vice-versa. \Kate{Tighten up language -- incomplete information and partial observability are specific technical terms, which would imply planning in belief space. You are not doing that. Simply say what agents know when. Again -- differentiate between generic and the specific}
The state for agent $f$, $s_{f} \in S$, is a one-hot vector of size $|\mathbf{T}|$ composed of all zeros but a one at index $\mathbf{t}_{o}$, the label of $o$'s team.
Agents are not made aware of their own team label, however must learn this through experience when interacting with their teammates.

\subsection{Opponent Sampling}
Prior work has found that cooperation can emerge when agents are able to change their social network~\cite{Pinheiro2012FromLT,Santos2020PickyLA,Anastassacos2020PartnerSF}, however this assumption is not always possible.\Kate{You don't really talk about social networks else where -- it is somewhat orthogonal to your problem. Just say you assume that it is possible for all agents to interact with each other. The issue is whether they are aware if they are intereacting with a teammate or someone from a different team (and if so, which one). What is important is that you are not letting them choose to partner with someone -- instead that match is made for them.}
Our model uses a stochastic sampling technique with a complete social graph so that $f$ is unable to explicitly choose their opponent.
% However, we do experiment with various probabilities over which team $o$ belongs to.
% Once a team is chosen by weighted random sampling, the specific agent who becomes $o$ is chosen with uniform probability.
% However, our model assumes some teams can be sampled with higher weight.
However, we define a variable $\alpha$ which affects the probability of $f$ sampling $o$ from within or outside of their own team.
This value is uniformly defined for all teams.
Let $t = \frac{1}{|\mathbf{T}|}$ and $\overline{t} = \frac{|\mathbf{T}| - 1}{|\mathbf{T}|}$ represent the probability, or frequency, of sampling $o$ from $\mathbf{t}_{f}$ and $\mathbf{T}^{-\mathbf{t}_{f}}$ respectively when all teams have equal probability.
The variable $\alpha$ makes $o \in \mathbf{t}_{f}$ more likely than any other team, and the probability of sampling $o$ from $\mathbf{T}^{-\mathbf{t}_{f}}$, calculated as $\overline{t} = 1 - \alpha t$,
% The weight $\alpha$ is used in the equation $(|\mathbf{T}| - 1) \alpha t = \overline{t}$ to determine the probability of sampling $o$ from $\mathbf{t}_{f}$ or $\mathbf{T}^{-\mathbf{t}_{f}}$.
is distributed evenly over the $|\mathbf{T}| - 1$ teams in $\mathbf{T}^{-\mathbf{t}_{f}}$.


% Less formally, when $\alpha > 1$ $o \in \mathbf{t}_{f}$ is the highest probability, $\alpha < 1$ means teams in $\mathbf{T}^{-\mathbf{t}_{f}}$ weighted heavier than $\mathbf{t}_{f}$, and $\alpha = 1$ means all teams are equally as likely to be chosen with a probability of $\frac{1}{|\mathbf{T}|}$ for all teams.
% % Note that equally as likely means a $\frac{1}{|\mathbf{T}|}$ probability of $o$ being on $\mathbf{t}_{f}$.
% Once a team is chosen, $o$ is sampled uniformly from $\mathbf{t}_{o}$ so that $Pr(o') = Pr(o'') \forall o', o'' \in \mathbf{t}_{o}$.




% For example, it may be the case that the probability of sampling an agent from the same team $P(\mathbf{t}_{f})$ is different than another team $P(\mathbf{t}_{o}) \in \mathbf{T}^{-\textbf{t}_{f}}$, however $P(o') = P(o'') \forall o', o'' \in \mathbf{t}_{o}$, each agent within the selected team has the same probability of being chosen.


\subsection{Learning and Optimization}
\Kate{If you set up a generic model -- this will already be covered. (ie the reward sharing). You are also having a lot of implementation details about the learning here which is not appropriate. That should all come later in the experimental section. The learning mechanism is irrelevant for any of the theoretical findings. }
To be consistent with the original work on teams, we assume teams are bounded by common-interest.
This is modeled in recent MARL work by reward sharing, thus teammates fully share rewards each episode, $r_{i} = \frac{1}{n} \sum_{\mathbf{j \in t_{i}}} r_{j}$ for any agent $i \in \mathbf{t}_{i}$.
Different from the original groundwork with teams, the agents in our experiments use neural networks to learn with more complexity than was previously possible.
To ensure agents remain heterogeneous, agents observe their own state $s_{i}$ and choose actions with and optimize their own policy $\pi_{i}$.
We avoid over-sharing beliefs, gradients, or optimization frameworks which is often used in centralized MARL algorithms, instead relying on teammates constructing coordinated policies through their own similar experiences.
% In this study, we do not allow for explicit communication between teammates although this could be added to improve team alignment in difference scenarios.
Our model of teams is purposefully general to allow for future work to expand on easily.
For example, sanctions, communication, and leadership groups are all characteristics of human behavior and teamwork which are easy to implement with our model.


\emph{Reputation} has a strong history in past work across many domains.
The notion of team reputation is important for our analysis, but we define reputation differently than previous work which uses a binary reputation signal~\cite{Xu2019CooperationWB,Santos2018SocialNC,Anastassacos2021CooperationAR}.

\begin{definition}
    %Team Reputation \\
    The \emph{reputation} of team $\mathbf{t}_{o}$ is how an agent $f$ \textbf{believes} $\mathbf{t}_{o}$ will act.
    This concept of reputation is constructed by all agents separately and is not explicitly stated or shared.
\end{definition}
\Kate{Is this definition something that you came up with yourself or is it from the literature.  How are capturing beliefs? Where do they come into play?}

Agents tracking the reputation of $\mathbf{t}_{o}$ instead of a reputation for $o$ is a result of partial observability since $n > 1$ is a requirement of our model.
Since the state space only contains team labels, we do not formally represent team reputation through separate mechanisms as in past work, although this could be added to our framework.
Instead, we define reputation as being equivalent to the internal beliefs, for example the Q values of Deep Q-Network agents, and base our theory on the actions agents are expected to take.
\Kate{The above paragraph will need to be rewritten -- you have not yet said much about the learning mechanism so far so it is coming out of the blue}

==> theory.tex <==
% \section{Theoretical Advantages of Teams}
\section{Equilibrium Analysis with Teams}
\label{sec:theory}

\todo{Could this be a subsubsection of the IPD section above? Or completely moved to the appendix.}



% We evaluate teams in the IPD and the Cleanup Markov game.
The underlying dynamics of Cleanup are reducible to a matrix social dilemma, therefore we analyze how the game-theoretical properties of the IPD matrix game are affected by various environmental parameters.
We consider the number of teams, distribution of interactions, and the costs and benefits of cooperation.
The extensive details of the derivation are given in Appendix B.

\input{eq_analysis}

% \input{team_theory}


